Are Pretrained Transformers Robust in Intent Classification? A Missing Ingredient in Evaluation of Out-of-Scope Intent Detection

Pre-trained Transformer-based models were reported to be robust in intent classification. In this work, we first point out the importance of in-domain out-of-scope detection in few-shot intent recognition tasks and then illustrate the vulnerability of pre-trained Transformer-based models against samples that are in-domain but out-of-scope (ID-OOS). We construct two new datasets, and empirically show that pre-trained models do not perform well on both ID-OOS examples and general out-of-scope examples, especially on fine-grained few-shot intent detection tasks. To figure out how the models mistakenly classify ID-OOS intents as in-scope intents, we further conduct analysis on confidence scores and the overlapping keywords, as well as point out several prospective directions for future work. Resources are available on https://github.com/jianguoz/Few-Shot-Intent-Detection.

==> related-works.tex <==
\section{Related Work}

Our work is related to text summarization tasks and generative adversarial networks (GANs). 

%\subsection{Text Summarization}
\textbf{Text Summarization.} In terms of text summarization, it mainly includes two categories of approaches: extractive and abstractive methods. Extractive methods produce a text summary by extracting and concatenating several words from original sentence. Whereas abstractive methods generate a text summary based on the original sentence, which usually generate more readable and coherent summaries. Traditional extractive methods such as  graphic models \cite{mihalcea2005language} and optimization-based models \cite{woodsend2010automatic} usually rely on human-engineered features. Recent RNN-based methods \cite{chopra2016abstractive,gong2018automatic,nallapati2017summarunner,wang2018multi} have become popular in text summarization tasks. 
Among them, \cite{gong2018automatic,wang2018multi} design attention-based neural networks for short product titles generation in E-commerce. \cite{gong2018automatic} considers rich semantic features of long product titles. \cite{wang2018multi} designs a multi-task model and uses user searching log data as additional task to facilitate key words extraction from original long titles. However, they mainly consider information from textual long product titles, which sometimes are not enough to select important words and filter out over-informative and irrelevant words from long product titles. In addition, these methods mainly apply MLE objective and predict next word based on previous words. As a consequence, these models usually suffer from \textit{exposure bias} and lack of human-like view.

\textbf{Generative Adversarial Networks (GANs)}.
GAN is firstly proposed in \cite{goodfellow2014generative}, which is designed for generating real-valued, continuous data, and has gained great success in computer vision tasks \cite{dai2017towards,isola2017image,ledig2017photo}.  However, applying GANs to discrete scenarios like natural language has encountered many difficulties, since the discrete elements break the differentiability of GANs and prohibit gradients backpropagating from the discriminator to generator. 
% Due to this reason, GAN has not achieved comparable success in NLP. Recently, researchers usually reformulate the problem to continuous domain or consider reinforcement learning problems. 
To mitigate these above mentioned issues, SeqGan \cite{yu2017seqgan} models sequence generation procedure as a sequential decision making process. It applies a policy gradient method to train the generator and discriminator, and shows improvements on multiple generation task such as poem generation and music generation. MaskGan \cite{fedus2018maskgan} designs a actor-critic reinforcement learning based GAN to improve qualities of text generation through filling in missing texts conditioned on the surrounding context. There are also some other RL based GANs for text generation such as LeakGan \cite{guo2017long}, RankGan \cite{lin2017adversarial}, SentiGan \cite{wang2018sentigan}, etc. All above methods are designed for unsupervised text generation tasks. 
\cite{li2017adversarial} designs an adversarial learning method for neural dialogue generation. They train a seq2seq model to produce responses and use a discriminator to distinguish whether the responses are human-generated and machine-generated, and showing promising results.
% They also propose some methods on how to stabilize training for GANs such as pretraining method. In this paper, we adopt their pretraining method before normal training process.  
It should be noticed that our work differs from other similar tasks such as image captioning \cite{dai2017towards} and visual question answering \cite{antol2015vqa}. The image captioning can be seen as generating caption from a single modality of input, while the visual question answering mainly focuses on aligning the input image and question to generate a correct answer. In our task, we put more attention on learning more information from the multi-modal input sources (i.e., long product titles, product image and attribute tags) to generate a short product title. 



==> tables_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{cl|ccc|ccc|ccc}
\hline
\multicolumn{1}{l}{\textbf{}} & \textbf{} & \multicolumn{3}{c|}{\textbf{In-scope accuracy}}           & \multicolumn{3}{c|}{\textbf{OOS recall}}                   & \multicolumn{3}{c}{\textbf{OOS precision}}                 \\
\multicolumn{2}{l|}{\textbf{5-shot}}      & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} \\ \hline
\multirow{4}{*}{ID-OOS}       & ALBERT    & 54.1 $\pm$ 6.9   & 55.5 $\pm$ 8.1        & 68.0 $\pm$ 3.7  & 86.3 $\pm$ 8.1   & 75.9 $\pm$ 11.2       & 89.9 $\pm$ 4.3  & 57.9 $\pm$ 3.3   & 55.8 $\pm$ 4.3        & 66.6 $\pm$ 2.5  \\
                              & BERT      & 75.2 $\pm$ 2.9   & 74.1 $\pm$ 4.6        & 83.2 $\pm$ 3.1  & 81.8 $\pm$ 10.5  & 76.5 $\pm$ 9.7        & 90.4 $\pm$ 5.6  & 70.8 $\pm$ 2.5   & 68.1 $\pm$ 3.2        & 79.5 $\pm$ 3.1  \\
                              & ELECTRA   & 64.8 $\pm$ 4.8   & 71.0 $\pm$ 7.3        & 83.3 $\pm$ 2.3  & 89.4 $\pm$ 4.3   & 75.8 $\pm$ 6.1        & 88.9 $\pm$ 3.9  & 65.1 $\pm$ 3.0   & 67.1 $\pm$ 4.8        & 79.6 $\pm$ 1.8  \\
                              & RoBERTa   & 83.8 $\pm$ 1.7   & 64.5 $\pm$ 5.6        & 88.5 $\pm$ 2.7  & 78.4 $\pm$ 6.2   & 86.8 $\pm$ 5.4        & 97.5 $\pm$ 3.1  & 78.6 $\pm$ 1.5   & 63.3 $\pm$ 3.4        & 85.7 $\pm$ 2.8  \\ %\cdashline{1-11}
                              \hdashline
\multirow{4}{*}{OOD-OOS}      & ALBERT    & 63.1 $\pm$ 5.7   & 55.5 $\pm$ 8.1        & 75.5 $\pm$ 3.5  & 85.3 $\pm$ 5.4   & 92.5 $\pm$ 4.0        & 87.3 $\pm$ 4.3  & 83.4 $\pm$ 1.7   & 81.5 $\pm$ 3.1        & 88.2 $\pm$ 1.4  \\
                              & BERT      & 75.2 $\pm$ 2.9   & 74.1 $\pm$ 4.6        & 83.2 $\pm$ 3.1  & 93.4 $\pm$ 3.7   & 95.5 $\pm$ 2.7        & 96.2 $\pm$ 1.2  & 88.8 $\pm$ 1.4   & 88.4 $\pm$ 1.9        & 92.2 $\pm$ 1.2  \\
                              & ELECTRA    & 75.5 $\pm$ 4.0   & 71.0 $\pm$ 7.3        & 83.3 $\pm$ 2.3  & 87.3 $\pm$ 4.3   & 87.6 $\pm$ 4.2        & 89.5 $\pm$ 2.8  & 88.8 $\pm$ 2.1   & 87.0 $\pm$ 2.7        & 91.8 $\pm$ 1.0  \\
                              & RoBERTa   & 83.8 $\pm$ 1.7   & 81.2 $\pm$ 4.0        & 88.5 $\pm$ 2.7  & 97.0 $\pm$ 0.9   & 96.7 $\pm$ 1.4        & 96.6 $\pm$ 1.1  & 92.9 $\pm$ 0.6   & 91.4 $\pm$ 1.8        & 94.4 $\pm$ 1.2  \\ \hline
\multicolumn{1}{l}{\textbf{}} & \textbf{} & \multicolumn{3}{c|}{\textbf{In-scope accuracy}}           & \multicolumn{3}{c|}{\textbf{OOS recall}}                   & \multicolumn{3}{c}{\textbf{OOS precision}}                 \\
%%%%%%%%%%%%%---10-Shot---%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{2}{l|}{\textbf{10-shot}}     & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} \\ \hline
\multirow{4}{*}{ID-OOS}       & Albert    & 77.8 $\pm$ 2.7   & 66.7 $\pm$ 7.8        & 81.5 $\pm$ 3.8  & 77.6 $\pm$ 13.0  & 79.8 $\pm$ 6.4        & 97.1 $\pm$ 2.8  & 72.2 $\pm$ 2.9   & 64.0 $\pm$ 4.1        & 78.9 $\pm$ 3.3  \\
                              & Bert      & 77.5 $\pm$ 1.7   & 80.3 $\pm$ 3.7        & 95.0 $\pm$ 1.5  & 87.5 $\pm$ 9.2   & 74.5 $\pm$ 6.9        & 94.7 $\pm$ 3.4  & 73.8 $\pm$ 1.7   & 73.1 $\pm$ 3.3        & 93.0 $\pm$ 2.0  \\
                              & Electra   & 79.5 $\pm$ 2.9   & 78.0 $\pm$ 2.5        & 93.2 $\pm$ 0.8  & 85.2 $\pm$ 9.1   & 86.5 $\pm$ 5.8        & 88.0 $\pm$ 4.5  & 75.4 $\pm$ 2.7   & 73.3 $\pm$ 2.9        & 90.3 $\pm$ 1.1  \\
                              & Roberta   & 76.6 $\pm$ 0.9   & 81.0 $\pm$ 5.5        & 94.3 $\pm$ 1.5  & 86.4 $\pm$ 6.3   & 83.9 $\pm$ 6.9        & 98.3 $\pm$ 1.9  & 72.7 $\pm$ 1.5   & 75.8 $\pm$ 5.2        & 92.4 $\pm$ 1.9  \\ \cdashline{1-11}
\multirow{4}{*}{OOD-OOS}      & Albert    & 77.8 $\pm$ 2.7   & 66.7 $\pm$ 7.8        & 88.6 $\pm$ 2.9  & 90.6 $\pm$ 4.0   & 95.0 $\pm$ 3.4        & 90.0 $\pm$ 2.5  & 89.8 $\pm$ 1.0   & 85.7 $\pm$ 2.7        & 94.3 $\pm$ 1.4  \\
                              & Bert      & 77.5 $\pm$ 1.7   & 90.1 $\pm$ 1.9        & 95.0 $\pm$ 1.5  & 96.8 $\pm$ 1.2   & 91.1 $\pm$ 4.4        & 91.4 $\pm$ 2.2  & 90.0 $\pm$ 0.7   & 95.5 $\pm$ 1.1        & 97.4 $\pm$ 0.7  \\
                              & Electra   & 79.5 $\pm$ 2.9   & 88.6 $\pm$ 2.1        & 93.2 $\pm$ 0.8  & 94.8 $\pm$ 1.7   & 89.1 $\pm$ 2.2        & 90.8 $\pm$ 3.2  & 90.7 $\pm$ 1.2   & 94.2 $\pm$ 1.1        & 96.5 $\pm$ 0.5  \\
                              & Roberta   & 89.2 $\pm$ 1.3   & 87.5 $\pm$ 3.3        & 94.3 $\pm$ 1.5  & 95.6 $\pm$ 1.0   & 94.6 $\pm$ 2.4        & 97.5 $\pm$ 1.0  & 95.4 $\pm$ 0.5   & 94.0 $\pm$ 1.4        & 97.2 $\pm$ 0.7  \\ \hline
\multicolumn{1}{l}{}          &           & \multicolumn{3}{c|}{\textbf{In-domain accuracy}}                    & \multicolumn{3}{c|}{\textbf{OOS recall}}                   & \multicolumn{3}{c}{\textbf{OOS precision}}                          \\
%%%%%%%%%%%%---10-Shot---%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{2}{l|}{\textbf{Full-shot}}            & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} \\ \hline
\multirow{4}{*}{ID-OOS}       & ALBERT    & 79.5 $\pm$ 3.0   & 86.5 $\pm$ 1.7        & 90.3 $\pm$ 3.0  & 73.4 $\pm$ 8.5   & 73.4 $\pm$ 3.9        & 96.3 $\pm$ 6.0  & 72.1 $\pm$ 3.9   & 79.4 $\pm$ 1.9        & 87.7 $\pm$ 3.1  \\
                              & BERT      & 89.4 $\pm$ 0.4   & 91.0 $\pm$ 0.4        & 96.6 $\pm$ 0.4  & 68.3 $\pm$ 6.4   & 70.4 $\pm$ 7.7        & 98.6 $\pm$ 0.1  & 82.8 $\pm$ 1.2   & 84.6 $\pm$ 1.7        & 95.5 $\pm$ 0.6  \\
                              & ELECTRA    & 92.8 $\pm$ 1.0   & 95.7 $\pm$ 0.6        & 97.6 $\pm$ 0.5  & 59.3 $\pm$ 2.6   & 65.5 $\pm$ 8.3        & 86.2 $\pm$ 5.8  & 87.0 $\pm$ 2.3   & 91.4 $\pm$ 1.0        & 96.1 $\pm$ 0.6  \\
                              & RoBERTa   & 92.2 $\pm$ 0.7   & 94.5 $\pm$ 0.7        & 96.7 $\pm$ 0.9  & 49.9 $\pm$ 2.5   & 51.9 $\pm$ 6.3        & 97.1 $\pm$ 1.0  & 83.4 $\pm$ 0.9   & 87.2 $\pm$ 1.5        & 95.4 $\pm$ 1.2  \\ %\cdashline{1-11}
                              \hdashline
\multirow{4}{*}{OOD-OOS}      & ALBERT    & 79.5 $\pm$ 3.0   & 86.5 $\pm$ 1.7        & 90.3 $\pm$ 3.0  & 96.0 $\pm$ 2.3   & 94.5 $\pm$ 2.4        & 94.8 $\pm$ 5.4  & 90.6 $\pm$ 1.3   & 93.4 $\pm$ 0.8        & 95.2 $\pm$ 1.3  \\
                              & BERT      & 89.4 $\pm$ 0.4   & 91.0 $\pm$ 0.4        & 96.6 $\pm$ 0.4  & 97.4 $\pm$ 0.6   & 99.0 $\pm$ 0.7        & 93.5 $\pm$ 1.6  & 95.2 $\pm$ 0.3   & 95.7 $\pm$ 0.2        & 98.3 $\pm$ 0.3  \\
                              & ELECTRA   & 92.8 $\pm$ 1.0   & 95.7 $\pm$ 0.6        & 97.6 $\pm$ 0.5  & 90.0 $\pm$ 3.4   & 94.7 $\pm$ 1.0        & 88.4 $\pm$ 3.1  & 96.7 $\pm$ 0.5   & 97.8 $\pm$ 0.3        & 98.6 $\pm$ 0.2  \\
                              & RoBERTa   & 92.2 $\pm$ 0.7   & 94.5 $\pm$ 0.7        & 96.7 $\pm$ 0.9  & 97.4 $\pm$ 0.7   & 93.6 $\pm$ 2.0        & 94.2 $\pm$ 2.1  & 96.6 $\pm$ 0.3   & 97.2 $\pm$ 0.2        & 98.3 $\pm$ 0.5  \\ \hline
\end{tabular}}
\caption{Testing results on the three different domains. \textcolor{red}{ADD `tod-bert-jnt-v1` and `ConvRT`. }}
\label{tb:main}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{cl|ccc|ccc|ccc}
\hline
\multicolumn{1}{l}{\textbf{}} & \textbf{} & \multicolumn{3}{c|}{\textbf{In-scope accuracy}}           & \multicolumn{3}{c|}{\textbf{OOS recall}}                   & \multicolumn{3}{c}{\textbf{OOS precision}}                 \\
\multicolumn{2}{l|}{\textbf{5-shot}}      &  \textbf{Banking} & \textbf{Credit cards} & \textbf{BANKING77-OOS} & \textbf{Banking} & \textbf{Credit cards} & \textbf{BANKING77-OOS} & \textbf{Banking} & \textbf{Credit cards} & \textbf{BANKING77-OOS} \\ \hline
\multirow{4}{*}{ID-OOS}       & ALBERT    & 54.1 $\pm$ 6.9   & 55.5 $\pm$ 8.1        &  20.3 $\pm$ 2.4 & 86.3 $\pm$ 8.1   & 75.9 $\pm$ 11.2       &  89.5 $\pm$ 1.5 & 57.9 $\pm$ 3.3   & 55.8 $\pm$ 4.3        &  39.8 $\pm$ 0.7 \\
                              & BERT      & 75.2 $\pm$ 2.9   & 74.1 $\pm$ 4.6        &  25.4 $\pm$ 3.6  & 81.8 $\pm$ 10.5  & 76.5 $\pm$ 9.7        & 90.9 $\pm$ 0.6  & 70.8 $\pm$ 2.5   & 68.1 $\pm$ 3.2        & 41.3 $\pm$ 1.4 \\
                              & ELECTRA   & 64.8 $\pm$ 4.8   & 71.0 $\pm$ 7.3        &  30.9 $\pm$ 2.3 & 89.4 $\pm$ 4.3   & 75.8 $\pm$ 6.1        & 87.5 $\pm$ 2.4  & 65.1 $\pm$ 3.0   & 67.1 $\pm$ 4.8        &  43.0 $\pm$ 0.8 \\
                              & RoBERTa   & 83.8 $\pm$ 1.7   & 64.5 $\pm$ 5.6        & 43.0 $\pm$ 2.9 & 78.4 $\pm$ 6.2   & 86.8 $\pm$ 5.4        & 83.1 $\pm$ 4.3 & 78.6 $\pm$ 1.5   & 63.3 $\pm$ 3.4        & 46.3 $\pm$ 1.9  \\ %\cdashline{1-11}
                              
                               & ToD-BERT   & 75.1 $\pm$ 2.3   & 67.4 $\pm$ 4.2      & 35.5 $\pm$ 1.5 & 75.8 $\pm$ 9.5   &    72.3 $\pm$ 3.4   & 82.7 $\pm$ 1.8 &  69.4 $\pm$ 3.6 & 61.3 $\pm$ 2.3     & 43.8 $\pm$ 0.1  \\ %\cdashline{1-11}
                              \hdashline
\multirow{4}{*}{OOD-OOS}      & ALBERT    & 63.1 $\pm$ 5.7   & 55.5 $\pm$ 8.1        & 20.3 $\pm$ 2.4  & 85.3 $\pm$ 5.4   & 92.5 $\pm$ 4.0        & 97.3 $\pm$ 2.5 & 83.4 $\pm$ 1.7   & 81.5 $\pm$ 3.1        &  39.9 $\pm$ 1.3 \\
                              & BERT      & 75.2 $\pm$ 2.9   & 74.1 $\pm$ 4.6        & 39.0 $\pm$ 3.1  & 93.4 $\pm$ 3.7   & 95.5 $\pm$ 2.7        & 94.1 $\pm$ 1.6  & 88.8 $\pm$ 1.4   & 88.4 $\pm$ 1.9        & 49.0 $\pm$ 1.8 \\
                              & ELECTRA    & 75.5 $\pm$ 4.0   & 71.0 $\pm$ 7.3        & 39.1 $\pm$ 2.7 & 87.3 $\pm$ 4.3   & 87.6 $\pm$ 4.2        & 93.1 $\pm$ 4.3 & 88.8 $\pm$ 2.1   & 87.0 $\pm$ 2.7        & 48.7 $\pm$ 1.1 \\
                              & RoBERTa   & 83.8 $\pm$ 1.7   & 81.2 $\pm$ 4.0        & 62.1 $\pm$ 2.9 & 97.0 $\pm$ 0.9   & 96.7 $\pm$ 1.4        & 93.9 $\pm$ 1.4 & 92.9 $\pm$ 0.6   & 91.4 $\pm$ 1.8        & 68.7 $\pm$ 2.2 \\
                              & ToD-BERT   & 83.0 $\pm$ 1.6   &  75.8 $\pm$ 5.0    & 52.9 $\pm$ 1.5 &  91.9 $\pm$ 1.0  &  96.7 $\pm$ 0.9     & 88.4 $\pm$ 1.7 & 92.8 $\pm$ 0.6  &  89.6 $\pm$ 2.1    & 66.0 $\pm$ 1.2 \\ %\cdashline{1-11}
                              \hline
\multicolumn{1}{l}{\textbf{10-shot}} & \textbf{} & \multicolumn{3}{c|}{}           & \multicolumn{3}{c|}{}                   & \multicolumn{3}{c}{}                  \\ \hline
%%%%%%%%%%%%%---10-Shot---%%%%%%%%%%%%%%%%%%%%%%%%
% \multicolumn{2}{l|}{\textbf{10-shot}}     & \textbf{Banking} & \textbf{Credit cards} & \textbf{BANKING77} & \textbf{Banking} & \textbf{Credit cards} & \textbf{BANKING77} & \textbf{Banking} & \textbf{Credit cards} & \textbf{BANKING77} \\ \hline
% \multicolumn{2}{l|}{\textbf{10-shot}}     &  & & & & &  &  &  & \\ \hline
\multirow{4}{*}{ID-OOS}       & ALBERT    & 77.8 $\pm$ 2.7   & 66.7 $\pm$ 7.8        &  27.3 $\pm$ 3.4 & 77.6 $\pm$ 13.0  & 79.8 $\pm$ 6.4        & 87.6 $\pm$ 1.3 & 72.2 $\pm$ 2.9   & 64.0 $\pm$ 4.1        & 42.4 $\pm$ 1.3  \\
% & ALBERT    & 77.8 $\pm$ 2.7   & 66.7 $\pm$ 7.8        &  27.3 $\pm$ 23.4 & 77.6 $\pm$ 13.0  & 79.8 $\pm$ 6.4        & 87.6 $\pm$ 11.3 & 72.2 $\pm$ 2.9   & 64.0 $\pm$ 4.1        & 42.4 $\pm$ 6.3  \\
                              & BERT      & 77.5 $\pm$ 1.7   & 80.3 $\pm$ 3.7        & 52.5 $\pm$ 1.7  & 87.5 $\pm$ 9.2   & 74.5 $\pm$ 6.9        & 77.3 $\pm$ 3.2  & 73.8 $\pm$ 1.7   & 73.1 $\pm$ 3.3        &   50.8 $\pm$ 1.1\\
                              & ELECTRA   & 79.5 $\pm$ 2.9   & 78.0 $\pm$ 2.5        & 40.1 $\pm$ 2.7  & 85.2 $\pm$ 9.1   & 86.5 $\pm$ 5.8        &  84.0 $\pm$ 1.7 & 75.4 $\pm$ 2.7   & 73.3 $\pm$ 2.9        & 46.1 $\pm$ 1.1   \\
                              & RoBERTa   & 76.6 $\pm$ 0.9   & 81.0 $\pm$ 5.5        & 59.7 $\pm$ 1.2  & 86.4 $\pm$ 6.3   & 83.9 $\pm$ 6.9        & 79.1 $\pm$ 1.7  & 72.7 $\pm$ 1.5   & 75.8 $\pm$ 5.2        &  55.8 $\pm$ 1.1 \\
                              & ToD-BERT   & 80.7 $\pm$ 2.5   &  80.6 $\pm$ 0.9    & 54.3 $\pm$ 1.8 &  79.5 $\pm$ 6.1  & 70.2 $\pm$ 5.9       & 76.9 $\pm$ 2.7 & 75.4 $\pm$ 1.4  & 71.9 $\pm$ 2.6      & 52.1 $\pm$ 1.2 \\ %\cdashline{1-11}
                              \cdashline{1-11}
\multirow{4}{*}{OOD-OOS}      & ALBERT    & 77.8 $\pm$ 2.7   & 66.7 $\pm$ 7.8        & 30.5 $\pm$ 6.5 & 90.6 $\pm$ 4.0   & 95.0 $\pm$ 3.4        &  92.7 $\pm$ 6.3 & 89.8 $\pm$ 1.0   & 85.7 $\pm$ 2.7        & 47.1 $\pm$ 1.9  \\
% & ALBERT    & 77.8 $\pm$ 2.7   & 66.7 $\pm$ 7.8        & 30.5 $\pm$ 26.5 & 90.6 $\pm$ 4.0   & 95.0 $\pm$ 3.4        &  92.7 $\pm$ 6.3 & 89.8 $\pm$ 1.0   & 85.7 $\pm$ 2.7        & 47.1 $\pm$ 11.9  \\
                              & BERT      & 77.5 $\pm$ 1.7   & 90.1 $\pm$ 1.9        & 64.2 $\pm$ 0.5 & 96.8 $\pm$ 1.2   & 91.1 $\pm$ 4.4        & 91.4 $\pm$ 3.2 & 90.0 $\pm$ 0.7   & 95.5 $\pm$ 1.1        & 68.9 $\pm$ 1.0  \\
                              & ELECTRA   & 79.5 $\pm$ 2.9   & 88.6 $\pm$ 2.1        & 40.1 $\pm$ 2.7  & 94.8 $\pm$ 1.7   & 89.1 $\pm$ 2.2        & 97.6 $\pm$ 1.0 & 90.7 $\pm$ 1.2   & 94.2 $\pm$ 1.1        &  47.9 $\pm$ 1.4 \\
                              & RoBERTa   & 89.2 $\pm$ 1.3   & 87.5 $\pm$ 3.3        & 70.3 $\pm$ 0.3 & 95.6 $\pm$ 1.0   & 94.6 $\pm$ 2.4        & 94.0 $\pm$ 0.8 & 95.4 $\pm$ 0.5   & 94.0 $\pm$ 1.4        & 73.3 $\pm$ 1.5 \\
                              & ToD-BERT   &  86.5 $\pm$ 2.6  &  86.5 $\pm$ 0.6   & 60.6 $\pm$ 1.8 & 96.0 $\pm$ 0.5   &  96.4 $\pm$ 0.5      & 94.9 $\pm$ 0.9 & 94.2 $\pm$ 1.2 &    93.7 $\pm$ 0.3 & 63.3 $\pm$ 0.9  \\ %\cdashline{1-11}
                              \hline
%%%%%%%%%%%%---10-Shot---%%%%%%%%%%%%%%%%%%%%%%%%%
% \multicolumn{1}{l}{}          &           & \multicolumn{3}{c|}{\textbf{In-domain accuracy}}                    & \multicolumn{3}{c|}{\textbf{OOS recall}}                   & \multicolumn{3}{c}{\textbf{OOS precision}}                          \\
% \multicolumn{2}{l|}{\textbf{Full-shot}}            & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} & \textbf{Banking} & \textbf{Credit cards} & \textbf{Travel} \\ \hline
% \multirow{4}{*}{ID-OOS}       & ALBERT    & 79.5 $\pm$ 3.0   & 86.5 $\pm$ 1.7        & 90.3 $\pm$ 3.0  & 73.4 $\pm$ 8.5   & 73.4 $\pm$ 3.9        & 96.3 $\pm$ 6.0  & 72.1 $\pm$ 3.9   & 79.4 $\pm$ 1.9        & 87.7 $\pm$ 3.1  \\
%                               & BERT      & 89.4 $\pm$ 0.4   & 91.0 $\pm$ 0.4        & 96.6 $\pm$ 0.4  & 68.3 $\pm$ 6.4   & 70.4 $\pm$ 7.7        & 98.6 $\pm$ 0.1  & 82.8 $\pm$ 1.2   & 84.6 $\pm$ 1.7        & 95.5 $\pm$ 0.6  \\
%                               & ELECTRA    & 92.8 $\pm$ 1.0   & 95.7 $\pm$ 0.6        & 97.6 $\pm$ 0.5  & 59.3 $\pm$ 2.6   & 65.5 $\pm$ 8.3        & 86.2 $\pm$ 5.8  & 87.0 $\pm$ 2.3   & 91.4 $\pm$ 1.0        & 96.1 $\pm$ 0.6  \\
%                               & RoBERTa   & 92.2 $\pm$ 0.7   & 94.5 $\pm$ 0.7        & 96.7 $\pm$ 0.9  & 49.9 $\pm$ 2.5   & 51.9 $\pm$ 6.3        & 97.1 $\pm$ 1.0  & 83.4 $\pm$ 0.9   & 87.2 $\pm$ 1.5        & 95.4 $\pm$ 1.2  \\ %\cdashline{1-11}
%                               \hdashline
% \multirow{4}{*}{OOD-OOS}      & ALBERT    & 79.5 $\pm$ 3.0   & 86.5 $\pm$ 1.7        & 90.3 $\pm$ 3.0  & 96.0 $\pm$ 2.3   & 94.5 $\pm$ 2.4        & 94.8 $\pm$ 5.4  & 90.6 $\pm$ 1.3   & 93.4 $\pm$ 0.8        & 95.2 $\pm$ 1.3  \\
%                               & BERT      & 89.4 $\pm$ 0.4   & 91.0 $\pm$ 0.4        & 96.6 $\pm$ 0.4  & 97.4 $\pm$ 0.6   & 99.0 $\pm$ 0.7        & 93.5 $\pm$ 1.6  & 95.2 $\pm$ 0.3   & 95.7 $\pm$ 0.2        & 98.3 $\pm$ 0.3  \\
%                               & ELECTRA   & 92.8 $\pm$ 1.0   & 95.7 $\pm$ 0.6        & 97.6 $\pm$ 0.5  & 90.0 $\pm$ 3.4   & 94.7 $\pm$ 1.0        & 88.4 $\pm$ 3.1  & 96.7 $\pm$ 0.5   & 97.8 $\pm$ 0.3        & 98.6 $\pm$ 0.2  \\
%                               & RoBERTa   & 92.2 $\pm$ 0.7   & 94.5 $\pm$ 0.7        & 96.7 $\pm$ 0.9  & 97.4 $\pm$ 0.7   & 93.6 $\pm$ 2.0        & 94.2 $\pm$ 2.1  & 96.6 $\pm$ 0.3   & 97.2 $\pm$ 0.2        & 98.3 $\pm$ 0.5  \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}}
\caption{Testing results on the ``Banking'' and ``Credit cards'' domains in CLINC-Single-Domain-OOS and BANKING77-OOS datasets.}
\label{tb:main}
% \vspace{-1.0em}
\end{table*}






% \begin{table}[]
% \begin{center}
%   \resizebox{1.0\linewidth}{!}{
% % {\small
% \begin{tabular}{ll}
% \hline
% Intent pair            & bill\_due \&     bill\_balance                                                                                                                                                                      \\ \hdashline
% Unigram overlap        & bill (60), pay (9), need (9), know (8), due (7)                                                                                                                                                     \\ \hdashline
% Matched ID-OOS example & \begin{tabular}[c]{@{}l@{}}i {[}mask{]} to {[}mask{]} what day i {[}mask{]} to {[}mask{]} \\ my water {[}mask{]}  $\rightarrow$ bill\_balance (confidence: \textbf{0.84})\end{tabular} \\ \hline
% Intent pair            & improve\_credit\_score \& credit\_score                                                                                                                                                             \\ \hdashline
% Unigram overlap        & credit (99), score (76), tell (7), want (3), like (3)                                                                                                                                               \\ \hdashline
% Matched ID-OOS example & \begin{tabular}[c]{@{}l@{}}i'd {[}mask{]} to make my {[}mask{]} {[}mask{]} better \\ $\rightarrow$ credit\_limit\_change (confidence: \textbf{0.86})\end{tabular}                     \\ \hline
% \end{tabular}}\caption{Examples investigated for the unigram overlap analysis. The overlap frequency is also shown.}\label{tb:word_overlap}
% \end{center}
% % \vspace{-1.9em}
% \end{table}



\begin{table*}[t]
  \begin{center}
  \resizebox{0.95\linewidth}{!}{
{\small
    \begin{tabular}{l|l|l}

    Intent pair              &   Unigram overlap              & Masked ID-OOS example sentence from the development set \\ \hline
    bill\_due      & bill (60), pay (9), need (9),  &  i [mask] to [mask] what day i [mask] to [mask] my water [mask] \\
    bill\_balance & know (8), due (7)              &  $\rightarrow$ bill\_balance (confidence: {\bf 0.84})   \\  \hdashline
    
    improve\_credit\_score      & credit (99), score (76), tell (7),  &  i'd [mask] to make my [mask] [mask] better \\
    credit\_score              & want (3), like (3)              &  $\rightarrow$ credit\_limit\_change (confidence: {\bf 0.86})   \\ \hline


    \end{tabular}}
}
    % \vspace{-0.5em}
    \caption{Examples investigated for the unigram overlap analysis. The overlap frequency is also shown.}
    \label{tb:word_overlap}
    % \vspace{-1.5em}
  \end{center}
\end{table*}

